Inverse obstacle scattering regularized by the tangent-point energy

We employ the so-called tangent-point energy as Tikhonov regularizer for ill-conditioned inverse scattering problems in 3D. The tangent-point energy is a self-avoiding functional on the space of embedded surfaces that also penalizes surface roughness. Moreover, it features nice compactness and continuity properties. These allow us to show the well-posedness of the regularized problems and the convergence of the regularized solutions to the true solution in the limit of vanishing noise level. We also provide a reconstruction algorithm of iteratively regularized Gauss-Newton type. Our numerical experiments demonstrate that our method is numerically feasible and effective in producing reconstructions of unprecedented quality.

==> Figure_Triceratops2.tex <==
% !TEX root = Main.tex

\begin{figure}[t]
	\centering
	\newcommand{\myheight}{0.31\textwidth}
	\newcommand{\inca}[2]{%
		\begin{tikzpicture}%
			\node[inner sep=0pt] (fig) at (0,0) {\includegraphics[	trim = 30 30 30 30, 
			clip = true,  
			angle = 0,
			height = \myheight]{#1}};%
			\node[above right= -0.125ex] at (fig.south west) {\begin{footnotesize}(#2)\end{footnotesize}};%
		\end{tikzpicture}%
	}%
	\inca{Figure_Triceratops/triceratops_BAEMM_16inc_TPM0_4pi6pi_remeshed/DistanceField}{a}%
	\hfill
	\inca{Figure_Triceratops/triceratops_BAEMM_16inc_TPM0_8pi_remeshed_new_tau_3_rho_0.8/DistanceField}{b}%
	\hfill
	\inca{Figure_Triceratops/triceratops_BAEMM_16inc_TPM0_8pi_remeshed_new_tau_3_rho_0.8/True_DistanceField}{c}%
	\hfill
	\includegraphics[trim = 0 0 0 0, 
	clip = true,  
	angle = 0,
	height = \myheight]{%
		Figure_Triceratops/triceratops_BAEMM_16inc_TPM0_8pi_remeshed_new_tau_3_rho_0.8/ColorBar
	}%
	\caption{%
		(a) Intermediate reconstruction of the Triceratops for wavelength $\lambda \in \braces{1/2,1/3}$, shaded by the signed distance field of the true obstacle.
		Some details are missing, in particular, between the two brown horns. 
		(b) Final reconstruction for $\lambda = 1/4$. 
		Now the wavelength is sufficiently small to separate the brow horns.
		(c) The signed distance field of (b), plotted on the true obstacle.
		It highlights the features that are particularly difficult to reconstruct.
	}%
	\label{fig:Triceratops2}
\end{figure}

==> Macros.tex <==
% !TEX root = Main.tex

\newcommand{\diffeo}{\varTheta}
\newcommand{\DirichletToNeumann}{\mathrm{DtN}}

\makeatletter
\newcommand\RedeclareMathOperator{%
  \@ifstar{\def\rmo@s{m}\rmo@redeclare}{\def\rmo@s{o}\rmo@redeclare}%
}
% this is taken from \renew@command
\newcommand\rmo@redeclare[2]{%
  \begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
  \expandafter\@ifundefined\@gtempa
     {\@latex@error{\noexpand#1undefined}\@ehc}%
     \relax
  \expandafter\rmo@declmathop\rmo@s{#1}{#2}}
% This is just \@declmathop without \@ifdefinable
\newcommand\rmo@declmathop[3]{%
  \DeclareRobustCommand{#2}{\qopname\newmcodes@#1{#3}}%
}
\@onlypreamble\RedeclareMathOperator
\makeatother

\DeclareDocumentCommand{\TProj}{ o }{
	\IfValueTF{#1}{
		P_{\!\smash{#1}}^\top
	}{
		P^\top
	}
}

\DeclareDocumentCommand{\NProj}{ o }{
	\IfValueTF{#1}{
		P_{\!\smash{#1}}^\perp
	}{
		P^\perp
	}
}


\newcommand{\DOpSymbol}{\mathcal{D}}
\newcommand{\dOpSymbol}{D}

\DeclareDocumentCommand{\DOp}{ o }{
	\IfValueTF{#1}{
		\mathop{}\!\DOpSymbol_{\!\smash{#1}}
	}{
		\mathop{}\!\DOpSymbol
	}
}

\newcommand{\DeltaOpSymbol}{\mathcal{D}}
\newcommand{\deltaOpSymbol}{D}

\DeclareDocumentCommand{\DeltaOp}{ o o }{
	\IfValueTF{#1}{
	  \IfValueTF{#2}{
        \mathop{}\!\DeltaOpSymbol^{\smash{(#1)}}_{\!\smash{#2}}
	  }{
        \mathop{}\!\DeltaOpSymbol^{\smash{(#1)}}
	  }
	}{
		\mathop{}\!\DeltaOpSymbol{\!\smash{#2}}
	}
}


\DeclareDocumentCommand{\deltaOp}{ o }{
	\IfValueTF{#1}{
		\mathop{}\!\deltaOpSymbol^{(#1)}
	}{
		\mathop{}\!\deltaOpSymbol
	}
}

\DeclareDocumentCommand{\DeltaOpG}{ o o }{
	\IfValueTF{#1}{
	  \IfValueTF{#2}{
        \mathop{}\!\underline{\DeltaOpSymbol}^{\smash{(#1)}}_{\!\smash{#2}}
	  }{
        \mathop{}\!\underline{\DeltaOpSymbol}^{\smash{(#1)}}
	  }
	}{
		\mathop{}\!\underline{\DeltaOpSymbol}_{\!\smash{#2}}
	}
}



\newcommand{\RemainderOpSymbol}{\mathcal{R}}
\newcommand{\remainderOpSymbol}{R}

\DeclareDocumentCommand{\RemainderOp}{ o o }{
	\IfValueTF{#1}{
	  \IfValueTF{#2}{
        \mathop{}\!\RemainderOpSymbol^{\smash{#1}}_{\!\smash{#2}}
	  }{
        \mathop{}\!\RemainderOpSymbol^{\smash{#1}}
	  }
	}{
		\mathop{}\!\RemainderOpSymbol_{\!\smash{#2}}
	}
}

\DeclareDocumentCommand{\RemainderOpG}{ o o }{
	\IfValueTF{#1}{
	  \IfValueTF{#2}{
        \mathop{}\!\underline{\RemainderOpSymbol}^{\smash{#1}}_{\!\smash{#2}}
	  }{
        \mathop{}\!\underline{\RemainderOpSymbol}^{\smash{#1}}
	  }
	}{
		\mathop{}\!\underline{\RemainderOpSymbol}_{\!\smash{#2}}
	}
}


\DeclareDocumentCommand{\remainderOp}{ o }{
	\IfValueTF{#1}{
		\mathop{}\!\remainderOpSymbol^{#1}
	}{
		\mathop{}\!\remainderOpSymbol
	}
}




\newcommand{\TaylorOpSymbol}{\mathcal{T}}
\newcommand{\taylorOpSymbol}{T}

\DeclareDocumentCommand{\TaylorOp}{ o o }{
	\IfValueTF{#1}{
	  \IfValueTF{#2}{
        \TaylorOpSymbol^{\smash{#1}}_{\!\smash{#2}}
	  }{
        \TaylorOpSymbol^{\smash{#1}}
	  }
	}{
		\TaylorOpSymbol{\!\smash{#2}}
	}
}

\DeclareDocumentCommand{\taylorOp}{ o }{
	\IfValueTF{#1}{
		\taylorOpSymbol^{#1}
	}{
		\taylorOpSymbol
	}
}


\newcommand{\GagliardoOp}[1]{\cA^{\smash{#1}}}
\newcommand{\GagliardoOpG}[1]{\underline{\cA}^{\smash{#1}}}
\newcommand{\gagliardoOp}[1]{A^{#1}}

\newcommand{\diffoffset}{\delta}



%\newcommand*{\R}{\mathbb{R}}
%\newcommand*{\N}{\mathbb{N}}
\newcommand*{\E}{\mathcal{E}}
\newcommand*{\M}{\mathcal{M}}
\newcommand*{\G}{\mathcal{G}}
%\newcommand*{\C}{\mathcal{C}}
\newcommand*{\W}{\mathcal{W}}
\newcommand*{\D}{\mathcal{D}}



\renewcommand*{\S}{\mathbb{S}}

\newcommand*{\wsp}{{W^{s,p}}}

\newcommand*{\der}{\mathrm{d}}
\newcommand*{\on}[1]{\operatorname{#1}}



\DeclareMathOperator{\atanh}{atanh}
%\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\im}{im}


\newcommand{\SoboSlobo}{Sobolev--Slobodeckij\xspace}
% \newcommand{\SoboSlobo}{Sobolev--Slobodecki\u{\i}\xspace}

\newcommand{\Obsolete}[1]{{\color{BurntOrange}{#1}}}
\newcommand{\CheckThis}[1]{{\color{BrickRed}{#1}}}

%\newcommand{\Id}{\on{I}}
\newcommand{\Id}{I}

\newcommand{\Frob}{\mathrm{F}}
\newcommand{\TP}{\mathrm{TP}}

\newcommand{\SO}{\mathrm{SO}}

\newcommand{\atlas}{\mathcal{A}}

\newcommand{\embeds}{\hookrightarrow}
\newcommand{\ConformalFactor}[2]{\pars[\big]{#1- \tfrac{\DomDim}{#2}}}

\newcommand{\Energy}{\cE}
\newcommand{\Metric}{\cG}
\newcommand{\Riesz}{\cM}
\newcommand{\Tikhonov}{\cJ}
% \newcommand{\Extension}{\cF}
\newcommand{\Extension}{\overline{D\Energy}}
\newcommand{\Tpr}{P^\top}
\newcommand{\Npr}{P^\perp}
\newcommand{\NumWaves}{N}

\DeclareMathOperator{\prx}{\pi_1}
\DeclareMathOperator{\pry}{\pi_2}

\newcommand{\Fourier}{\mathscr{F}}

\newcommand{\Angle}[2]{\measuredangle(#1,#2)}
\newcommand{\bigAngle}[2]{\measuredangle \big( #1,#2 \big)}
\newcommand{\BigAngle}[2]{\measuredangle \Big( #1,#2 \Big)}


\newcommand{\OpenBall}[2]{B(#1;#2)}
\newcommand{\ClosedBall}[2]{\bar B(#1;#2)}
\newcommand{\bigClosedBall}[2]{\bar B \,\pars[\big]{#1;#2}}
\newcommand{\BigClosedBall}[2]{\bar B \,\pars[\Big]{#1;#2}}

\newcommand{\AmbDim}{m} % dimension of ambient space
\newcommand{\AmbSpace}{{\R^\AmbDim}}

\newcommand{\DomDim}{n} % dimension of domain 
\newcommand{\DomSpace}{{\R^\DomDim}}
\newcommand{\Domain}{M}
\newcommand{\IInt}{\int_\Domain \! \int_\Domain}

\newcommand{\NormalSpace}{\R^{\AmbDim-\DomDim}}

\newcommand{\TargetSpace}{H}

\newcommand{\Sphere}{\mathbb{S}}
\newcommand{\Disk}{\mathbb{B}}
\newcommand{\Ball}{\Disk}
\newcommand{\UnitTangent}{\operatorname{UT}}
\newcommand{\TangentBundle}{T}

\newcommand{\ContOps}{\cL}

\DeclareDocumentCommand{\Hess}{ O{} }{\operatorname{Hess}_{#1}}

\newcommand{\nospaceperiod}{\makebox[0pt][l]{\,.}}
\newcommand{\nospacecomma}{\makebox[0pt][l]{\,.}}


\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\Mean}{\operatorname{Mean}}
	
\newcommand{\qand}{\quad \text{and} \quad}
\newcommand{\qqand}{\qquad \text{and} \qquad}
\newcommand{\qwith}{\quad\text{with}\quad}
\newcommand{\qwhere}{\quad\text{where}\quad}
\newcommand{\qforall}{\quad\text{forall}\quad}

\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\Lip}{Lip}


\ifthenelse{\isundefined{\transp}}{\newcommand{\transp}{{\mathsf{T}}}}{}
\newcommand{\adj}{^{*}}
\newcommand{\dual}{'}
\newcommand{\ddual}{''}
\newcommand{\pinv}{^{\dagger}}

\newcommand{\mymathcal}{\mathcal}

\newcommand{\cA}{{\mymathcal{A}}}
\newcommand{\cB}{{\mymathcal{B}}}
\newcommand{\cC}{{\mymathcal{C}}}
\newcommand{\cD}{{\mymathcal{D}}}
\newcommand{\cE}{{\mymathcal{E}}}
\newcommand{\cF}{{\mymathcal{F}}}
\newcommand{\cG}{{\mymathcal{G}}}
\newcommand{\cH}{{\mymathcal{H}}}
\newcommand{\cI}{{\mymathcal{I}}}
\newcommand{\cJ}{{\mymathcal{J}}}
\newcommand{\cK}{{\mymathcal{K}}}
\newcommand{\cL}{{\mymathcal{L}}}
\newcommand{\cM}{{\mymathcal{M}}}
\newcommand{\cN}{{\mymathcal{N}}}
\newcommand{\cO}{{\mymathcal{O}}}
\newcommand{\cP}{{\mymathcal{P}}}
\newcommand{\cQ}{{\mymathcal{Q}}}
\newcommand{\cR}{{\mymathcal{R}}}
\newcommand{\cS}{{\mymathcal{S}}}
\newcommand{\cT}{{\mymathcal{T}}}
\newcommand{\cU}{{\mymathcal{U}}}
\newcommand{\cV}{{\mymathcal{V}}}
\newcommand{\cW}{{\mymathcal{W}}}
\newcommand{\cX}{{\mymathcal{X}}}
\newcommand{\cY}{{\mymathcal{Y}}}
\newcommand{\cZ}{{\mymathcal{Z}}}

%\newcommand{\SO}{\operatorname{SO}}

\newcommand{\co}{\colon \!\!}


\DeclareMathOperator{\Laplacian}{\Delta}
%\newcommand{\dd}{{\operatorname{d}}}
\newcommand{\dd}{\mathop{}\!\mathrm{d}}

\newcommand{\at}{|}
\newcommand{\At}{\big|}



\newcommand{\ii}{{\mathrm{i}}}
\newcommand{\jj}{{\mathrm{j}}}
\newcommand{\kk}{{\mathrm{k}}}
\newcommand{\ee}{{\mathrm{e}}}
\newcommand{\lamda}{{\lambda}}
\newcommand{\vu}{{\nu}}
\newcommand{\ceq}{\coloneqq}
\newcommand{\qec}{\eqqcolon}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\C}{{\mathbb{C}}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{{\mathbb{Z}}}
\newcommand{\Q}{{\mathbb{Q}}}
\newcommand{\HH}{{\mathbb{H}}}
\newcommand{\PP}{{\mathbb{P}}}
\newcommand{\K}{{\mathbb{K}}}
\newcommand{\F}{{\mathbb{F}}}

\DeclareMathOperator{\id}{id}


\newcommand{\scale}{\operatorname{sc}}
\newcommand{\stereo}{\operatorname{st}}

% {〈pre code〉} {〈left_delim〉} {〈right_delim〉} {〈post code〉} {〈body〉}
\DeclarePairedDelimiterXPP{\pars}[1]{\mathop{}}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\abs}[1]{\mathop{}}{\lvert}{\rvert}{}{#1}
\DeclarePairedDelimiterXPP{\norm}[1]{\mathop{}}{\lVert}{\rVert}{}{#1}
\DeclarePairedDelimiterXPP{\seminorm}[1]{\mathop{}}{\lbrack}{\rbrack}{}{#1}
\DeclarePairedDelimiterXPP{\inner}[1]{\mathop{}}{\langle}{\rangle}{}{#1}
\DeclarePairedDelimiterXPP{\iinner}[1]{\mathop{}}{\langle\!\langle}{\rangle\!\rangle}{}{#1}
\DeclarePairedDelimiterXPP{\brackets}[1]{\mathop{}}{\lbrack}{\rbrack}{}{#1}
\DeclarePairedDelimiterXPP{\braces}[1]{\mathop{}}{\lbrace}{\rbrace}{}{#1}

\DeclarePairedDelimiterXPP{\floor}[1]{\mathop{}}{\lfloor}{\rfloor}{}{#1}
\DeclarePairedDelimiterXPP{\ceil}[1]{\mathop{}}{\lceil}{\rceil}{}{#1}

\DeclarePairedDelimiterXPP{\intervalcc}[1]{\mathop{}}{\lbrack}{\rbrack}{}{#1}
\DeclarePairedDelimiterXPP{\intervalco}[1]{\mathop{}}{\lbrack}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP{\intervaloc}[1]{\mathop{}}{\lparen}{\rbrack}{}{#1}
\DeclarePairedDelimiterXPP{\intervaloo}[1]{\mathop{}}{\lparen}{\rparen}{}{#1}

\DeclarePairedDelimiterXPP{\myset}[2]{\mathop{}}{\lbrace}{\rbrace}{}{#1\,\delimsize\vert\,\mathopen{}#2}


% % \DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
% % \DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
% % \DeclarePairedDelimiter{\seminorm}{[}{]}
% % \DeclarePairedDelimiter{\inner}{\langle}{\rangle}
% % \DeclarePairedDelimiter{\brackets}{[}{]}
% % \DeclarePairedDelimiter{\braces}{\lbrace}{\rbrace}

% % \let\set\undefined
% % \let\Set\undefined
% % \DeclarePairedDelimiterX{\set}[2]{\lbrace}{\rbrace}{#1\,\delimsize\vert\,\mathopen{}#2}

% % \DeclarePairedDelimiter{\intervalcc}{[}{]}
% % \DeclarePairedDelimiter{\intervalco}{[}{[}
% % \DeclarePairedDelimiter{\intervaloc}{]}{]}
% % \DeclarePairedDelimiter{\intervaloo}{]}{[}

% \DeclarePairedDelimiter{\intervalcc}{[}{]}
% \DeclarePairedDelimiter{\intervalco}{[}{)}
% \DeclarePairedDelimiter{\intervaloc}{(}{]}
% \DeclarePairedDelimiter{\intervaloo}{(}{)}

% \DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
% \DeclarePairedDelimiter{\ffloor}{\lfloor\!\lfloor}{\rfloor\!\rfloor}
% \DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

% %Frobenius norm
% \DeclarePairedDelimiter{\fnorm}{\lvert}{\rvert}

% %Frobenius inner product
% % \DeclarePairedDelimiter{\finner}{\langle}{\rangle_\Frob}
% \DeclarePairedDelimiter{\finner}{\langle}{\rangle}

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Imag}{{\mathfrak{Im}}}
\DeclareMathOperator{\Real}{{\mathfrak{Re}}}
\DeclareMathOperator{\Ima}{im}
\DeclareMathOperator{\ima}{im}
\DeclareMathOperator{\Aut}{Aut}
\RedeclareMathOperator{\supp}{supp}   %support
\DeclareMathOperator{\diam}{diam}  %Diameter
\DeclareMathOperator{\dist}{dist}  %Distance
\DeclareMathOperator{\End}{End}    %Endomorphisms
\DeclareMathOperator{\Hom}{Hom}    %Homomorphisms
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\pr}{\pi}
\DeclareMathOperator{\grad}{grad}  
\DeclareMathOperator{\diver}{div}  
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\vol}{{\omega}}
\newcommand{\dvol}{\dd \omega}

\newcommand{\pull}{\#}
\newcommand{\push}{\#}

\newcommand{\Span}{\mathrm{span}}
\newcommand{\Stab}{\mathrm{stab}}
\newcommand{\lot}{\mathrm{l.o.t.{}}}

\newcommand{\fX}{{\mathfrak{X}}}
\newcommand{\fY}{{\mathfrak{Y}}}

\newcommand{\HsdM}{\mathcal{H}}
\newcommand{\HsdD}{d_\cH}


\newcommand{\Av}{\on{Av}}
\newcommand{\Mass}{\on{Mass}}

\newcommand{\scat}{{\mathrm{s}}}
\newcommand{\inc}{{\mathrm{i}}}
\newcommand{\loc}{{\mathrm{loc}}}
\newcommand{\bounded}{{\mathrm{b}}}

\DeclareDocumentCommand{\converges}{ o }{
	\mathbin{%
		\IfValueTF{#1}{%
			\mathrel{\vbox{\offinterlineskip\ialign{%
				\hfil##\hfil\cr
				$\scriptscriptstyle#1$\cr
				%\noalign{\kern0ex}
				$-\!\!\!-\!\!\!\rightarrow$\cr
			}}}
		}{%
			-\!\!\!-\!\!\!\rightarrow
		}%
	}%
}

\DeclareDocumentCommand{\wconverges}{ o }{
	\mathbin{%
		\IfValueTF{#1}{%
			\mathrel{\vbox{\offinterlineskip\ialign{%
				\hfil##\hfil\cr
				$\scriptscriptstyle#1$\cr
				%\noalign{\kern0ex}
				$-\!\!\!-\!\!\!\rightharpoonup$\cr
			}}}
		}{%
			-\!\!\!-\!\!\!\rightharpoonup
		}%
	}%
}

\DeclareDocumentCommand{\Measure}{ o }{
	\IfValueTF{#1}{%
		\mu_{\!#1}
	}{%
		\mu
	}%
}

% from https://www.grputland.com/2015/02/fine-control-over-sizes-of-fractions-in-latex.html
\newcommand{\sdfrac}[2]{\mbox{\small$\displaystyle\frac{#1}{#2}$}}
\newcommand{\fdfrac}[2]{\mbox{\footnotesize$\displaystyle\frac{#1}{#2}$}}
\newcommand{\ltfrac}[2]{\mbox{\large$\frac{#1}{#2}$}}
